Dissecting adaptive methods in GANs

Adaptive methods are a crucial component widely used for training generative adversarial networks (GANs). While there has been some work to pinpoint the "marginal value of adaptive methods" in standard tasks, it remains unclear why they are still critical for GAN training. In this paper, we formally study how adaptive methods help train GANs; inspired by the grafting method proposed in arXiv:2002.11803 [cs.LG], we separate the magnitude and direction components of the Adam updates, and graft them to the direction and magnitude of SGDA updates respectively. By considering an update rule with the magnitude of the Adam update and the normalized direction of SGD, we empirically show that the adaptive magnitude of Adam is key for GAN training. This motivates us to have a closer look at the class of normalized stochastic gradient descent ascent (nSGDA) methods in the context of GAN training. We propose a synthetic theoretical framework to compare the performance of nSGDA and SGDA for GAN training with neural networks. We prove that in that setting, GANs trained with nSGDA recover all the modes of the true distribution, whereas the same networks trained with SGDA (and any learning rate configuration) suffer from mode collapse. The critical insight in our analysis is that normalizing the gradients forces the discriminator and generator to be updated at the same pace. We also experimentally show that for several datasets, Adam's performance can be recovered with nSGDA methods.

==> old_num_exp.tex <==
\vspace{-3mm}

\section{Numerical performance of nSGDA}\label{sec:num_exp}
%\vspace{-3mm}



\autoref{sec:motivation} indicates that nSGDA may work as well as Adam in GAN training. In this section, we empirically verify this hypothesis through an extensive numerical study. To evaluate the proposed algorithm, we conducted extensive
experiments on CIFAR-10 \citep{krizhevsky2009learning}, LSUN Churches \citep{yu2016lsun}, STL-10 \citep{coates2011analysis} and Celeba-HQ \citep{liu2015faceattributes}. 
Similarly to above, we choose the Fr\'{e}chet Inception distance (FID) \citep{heusel2017gans} to quantitatively assess the performance of the model.  In all our experiments, 50k samples are randomly generated for each model to compute the FID. As for the architectures, we choose Resnets \citep{he2016identity} from \cite{gidel2018variational} and set up the WGAN-GP loss \citep{gulrajani2017improved}. Note that for each optimizer, we grid-search over stepsizes to find the best one in terms of FID. Due to limited computational resources, we trained the models for 100 epochs in the case of CIFAR-10 and Celeba-HQ and for 50 epochs for LSUN and STL-10. We apply a linear decay learning rate scheduling during training. Results are averaged over 10 seeds.

 
%In \autoref{sec:app_exp}, results when using DCGAN can also be found.

%\subsection{nSGDA competes with Adam}








\begin{wrapfigure}[18]{r}{0.48\textwidth}
\vspace{-.7cm}
  %\begin{center}
    %\includegraphics[width=0.48\textwidth]{birds}
       \centering
       %      \hspace{2.cm}
         \includegraphics[width=.9\linewidth]{images/batch_tmp.png}
       %  \vspace{-.3cm}
       % \caption*{(d)}
        \label{fig:batchcifar_final}
%   \end{minipage} 
 \vspace{-5mm}
\caption{\small FID score of a Resnet WGAN-GP model trained with l-nSGDA, g-nSGDA, Adam, and SGDA against the batch size in the CIFAR-10 dataset. At small batch sizes, the best performing models are those trained with nSGDA methods. As the batch size increases, the performance of nSGDA methods worsens and Adam performs better. Lastly, models trained with nSGDA consistently outperform those trained with SGDA. }\label{fig:batch plots}
\vspace{-.3cm}
\end{wrapfigure}
\textbf{nSGDA competes with Adam.} 
\autoref{fig:final plots} shows the performance of l-nSGDA, g-nSGDA, Adam, and SGD on different datasets. We first observe that l-nSGDA and g-nSGDA compete with Adam in all these datasets. On the other hand, SGD struggles to produce good quality images compared to the other methods as expected. It is worth reminding that the nSGDA methods and SGD have the \emph{same direction} but \emph{differ in their magnitude}.  Therefore, this experiment confirms our hypothesis that adaptive methods outperform SGDA thanks to their implicit step-size schedule. Lastly, we highlight that l-nSGDA and g-nSGDA perform almost as well. This suggests that a global step-size adaptivity is enough to perform well in GANs. Similar observations hold for DCGAN (see \autoref{sec:app_exp}). %These observations also hold for other architectures such as DCGAN (see \autoref{sec:app_exp}).
%We train a WGAN-GP using Adam, nSGDA and global nSGDA (g-nSGDA). This latter is a variant that consists in a nSGDA update where instead of dividing by the norm of the gradient with respect to a parameter, we divide by the sum of the norms of the gradient with respect to each parameter in the network. The reason we also consider g-nSGDA is to understand whether the needed adaptivity is local or global.


%\autoref{fig:final plots} shows that on different datasets, the normalized SGDA methods compete with Adam. Besides, we observe that we do not need a parameter-wise adaptivity since g-nSGDA performs as well as nSGDA. Images generated by these trained models can be found in \autoref{sec:app_exp}. We also confirm that the  normalized SGDA methods compete with Adam in other architectures such as DCGAN. Numerical results in this direction can also be found in \autoref{sec:app_exp}. 
%{sec:app_exp}
%  \begin{figure}[tbp] 
%   \vspace{-.5cm}

% % \begin{minipage}{0.45\textwidth}

% \vspace{-6mm}
% \end{figure}

\begin{figure*}[tbp]
 \begin{subfigure}{0.245\textwidth}
       %\hspace{-.4cm}
         \includegraphics[width=1.\linewidth]{images/cifar10_tmp.png} 
     %    \vspace{-.3cm}
        \caption*{(a) CIFAR-10}
        \label{fig:cifar10_final}
    \end{subfigure}
 \begin{subfigure}{0.245\textwidth}
       
        %    \hspace{1.cm}
         \includegraphics[width=1.\linewidth]{images/lsun_tmp.png}
       %  \vspace{-.3cm}
        \caption*{(b) LSUN Churches}
        \label{fig:lsun_final}
    \end{subfigure}
 \begin{subfigure}{0.245\textwidth}
       
             %\hspace{1.cm}
         \includegraphics[width=1.\linewidth]{images/stl10_tmp.png}
       %  \vspace{-.3cm}
        \caption*{(c) STL-10}
        \label{fig:stl10_final}
    \end{subfigure} 
 \begin{subfigure}{0.245\textwidth}
       
             %\hspace{1.cm}
         \includegraphics[width=1.\linewidth]{images/celeba_tmp.png}
       %  \vspace{-.3cm}
        \caption*{(d) Celeba-HQ}
        \label{fig:celeba_final}
    \end{subfigure} 
\caption{\small 
FID scores obtained when training a Resnet WGAN-GP using Adam, l-nSGDA, g-nSGDA, and SGD on different datasets. In all these datasets, l-nSGDA, g-nSGDA and Adam perform approximately as well. SGDA performs much worse.}\label{fig:final plots}
\vspace{-3mm}
\end{figure*}

%\subsection{Influence of the batch size}

\textbf{Influence of batch size.} While the nSGDA methods compete with Adam in GAN, it remains unclear whether such performance is proper to the algorithm or tied to the stochastic noise of the gradients. \autoref{fig:batch plots} shows the performance of the model trained with l-nSGDA, g-nSGDA, Adam, and SGD and using a wide range of batch sizes. We remark that the nSGDA methods perform better than Adam when the batch size is small. However, as the batch size increases, their performance seriously deteriorates. On the other hand, the performance of Adam seems to be less sensitive to the change of batch size. As expected, SGD overall performs poorly. nSGDA performs well in a relevant batch-size regime, as many GAN architectures such as DCGAN, WGAN-GP, SNGAN \citep{miyato2018spectral}, SAGAN \citep{zhang2019self} requires small batch sizes for optimal performances.
% To this end, we train a WGAN-GP on CIFAR-10 on a wide range of batch sizes. \autoref{fig:batch plots} shows the performance of the model trained with nSGDA, g-nSGDA, Adam and SGD. As expected, SGD generalizes overall poorly. We remark that the methods with SGD direction i.e. nSGDA, g-nSGDA and SGD perform better when the batch size is small. Their performance seriously deteriorates when the batch size is large. On the other hand, Adam generalizes poorly at extreme batch sizes i.e. at 8 and 512. However, we remark that at large batch sizes, Adam performs better than nSGDA and SGD. Therefore, we hypothesize that the generalization benefits of nSGDA is tied to the stochastic gradient. Note that most of the popular GAN architectures such DCGAN, WGAN-GP, SNGAN \citep{miyato2018spectral}, SAGAN \citep{zhang2019self} use small batch sizes which matches with the regime where nSGDA is effective.

